SpReME: Sparse Regression for Multi-Environment Dynamic Systems

Learning dynamical systems is a promising avenue for scientific discoveries. However, capturing the governing dynamics in multiple environments still remains a challenge: model-based approaches rely on the fidelity of assumptions made for a single environment, whereas data-driven approaches based on neural networks are often fragile on extrapolating into the future. In this work, we develop a method of sparse regression dubbed SpReME to discover the major dynamics that underlie multiple environments. Specifically, SpReME shares a sparse structure of ordinary differential equation (ODE) across different environments in common while allowing each environment to keep the coefficients of ODE terms independently. We demonstrate that the proposed model captures the correct dynamics from multiple environments over four different dynamic systems with improved prediction performance.

==> tex/preliminaries.tex <==
% : 우리 방법이 SINDy를 base로 하는 부분이 많으니까 여기에 대해서만 설명?
\section{Preliminary}
In this section, we describe the details of the sparse identification of nonlinear dynamics (SINDy)~\cite{SINDy} algorithm served as a baseline model in our work.


We consider nonlinear dynamical systems formalized as
\begin{equation}
\label{eqn:problem_setting}
    \frac{d\B{x}(t)}{dt}=f(\B{x}(t)),
\end{equation}
where $\B{x}(t)=[x_1(t), \cdots, x_n(t)]\in\mathbb{R}^{1\times n}$ represents $n$-dimensional state of the system at time $t$, and function $f(\cdot)$ describes a motion of the system.
Under the assumption that the function $f$ consists of only a few terms, SINDy casts the problem of uncovering dynamics into a problem of solving a sparse regression problem.

Let $\B{X}=[\B{x}(t_1);\B{x}(t_2);\cdots;\B{x}(t_m)]\in\mathbb{R}^{m\times n}$ and $\dot{\B{X}}=[d\B{x}(t_1)/dt;d\B{x}(t_2)/dt;\cdots;d\B{x}(t_m)/dt]\in\mathbb{R}^{m\times n}$ be a sequence of observations from $m$ different time steps and their derivatives, respectively. \st{The finite difference method is utilized to obtain the derivative of $\dot{\B{X}}$ when $\B{X}$ is available. To mitigate differentiation error, the total variation regularization technique is implemented~\cite{Chartrand2011}.}
%Our method is based on the sparse identification of nonlinear dynamics (SINDy)~\cite{SINDy} algorithm. 
%SINDy aims to discover unknown function $f(\cdot)$
%when $m$ time stamps of state $\B{X}=[\B{x}(t_1);\B{x}(t_2);\cdots;\B{x}(t_m)]\in\mathbb{R}^{m\times n}$ and its derivative $\dot{\B{X}}=[d\B{x}(t_1)/dt;d\B{x}(t_2)/dt;\cdots;d\B{x}(t_m)/dt]\in\mathbb{R}^{m\times n}$ are given.
Given a set of $p$ non-linear feature functions $\phi_i:\mathbb{R}^{m\times n} \rightarrow \mathbb{R}^{m \times 1}$, SINDy constructs a data matrix $\Phi(\B{X})=[\phi_1(\B{X});\phi_2(\B{X});\cdots;\phi_p(\B{X})]\in\mathbb{R}^{m\times p}$, where each column represents a candidate non-linear function. % which contains the $p$ feature function $\phi_i(\B{X})\in\mathbb{R}^{m\times 1}$.
%Each feature function represents a candidate of the dynamic $f(\cdot)$'s composition.
% The design of $\phi(x)$ is based on prior knowledge. 
%For example, $\Phi(\B{X})$ may form like $[1, x_1(t), x_2(t), x_1(t)x_2(t), \sin(x_1(t)), \sin(x_2(t))]$, when $n=2$ and $m=1$.
SINDy models the dynamics discovery as a sparse regression problem
\begin{equation}\label{eq:LR_form_of_SINDy}
    \dot{\B{X}} = \Phi(\B{X}) \B{\Xi},
\end{equation}
where $\B{\Xi}\in\mathbb{R}^{p\times n}$ represents a set of sparse coefficient.

%Value of the coefficient's element can dismiss the candidate by setting its corresponding elements as zero.
%In more detail, $(\Xi)_{i,j}=0$ represents that a derivative of state $\frac{d}{dt}x_j(t)$ does not consist of a candidate $\phi_i(\B{X})$.
% The algorithm performs sparse linear regression to extract meaningful and simple dynamics.
% feature function을 통해 dynamics를 구성할 nonlinear function의 후보군을 construct함으로써, SINDy는 dynamics discovery 문제를 nonlinear candidate과 state의 미분값 사이의 sparse linear regression 문제로 변환한다.
%SINDy assumes that the dynamics is constructed with few terms, to be the simplest structure.
%Under the assumption, which holds for many systems, SINDy prefers sparse structure for $\B{\Xi}$.

To find a sparse structure of $\B{\Xi}$, SINDy iterates over optimization and pruning steps alternatively.
During the optimization step, mean-squared-error (MSE) loss with $\ell_1$ regularization term is used to minimize the following objective:
% The loss function for training $\xi$:
\begin{equation} \label{eqn:SINDy_loss}
    \min_{\Xi} \norm{\dot{\B{X}}-\Phi(\B{X}) \B{\Xi}}_2^2 + \lambda\norm{\B{\Xi}}_1,
\end{equation}
where hyperparameter $\lambda$ controls the strength of the regularization term.
During the pruning step, the coefficients whose absolute values are smaller than a predetermined threshold are set to zero. Once the coefficients are pruned, they are not optimized in the further steps.

Note that the choice of the feature functions is important since the feature functions are the candidate terms to form the dynamic equation. Although, in the original work, constant, polynomial, and trigonometric feature functions are used as candidates, with prior knowledge of dynamic systems, one can choose a proper set of candidates that can potentially explain the dynamic systems well.


% and prunes elements of $\Xi$ to extract meaningful and simple dynamics.

% $\lambda$ is hyperparameter.
% L1-norm derives sparse $\xi$.
% We can apply various optimization techniques like LASSO, gradient descent, etc.
% By optimizing the loss function, we can find meaningful and simple dynamics.
